Tag-based regulation of modules in genetic programming improves context-dependent problem solving

We introduce and experimentally demonstrate the utility of tag-based genetic regulation, a new genetic programming (GP) technique that allows programs to dynamically adjust which code modules to express. Tags are evolvable labels that provide a flexible mechanism for referencing code modules. Tag-based genetic regulation extends existing tag-based naming schemes to allow programs to "promote" and "repress" code modules in order to alter expression patterns. This extension allows evolution to structure a program as a gene regulatory network where modules are regulated based on instruction executions. We demonstrate the functionality of tag-based regulation on a range of program synthesis problems. We find that tag-based regulation improves problem-solving performance on context-dependent problems; that is, problems where programs must adjust how they respond to current inputs based on prior inputs. Indeed, the system could not evolve solutions to some context-dependent problems until regulation was added. Our implementation of tag-based genetic regulation is not universally beneficial, however. We identify scenarios where the correct response to a particular input never changes, rendering tag-based regulation an unneeded functionality that can sometimes impede adaptive evolution. Tag-based genetic regulation broadens our repertoire of techniques for evolving more dynamic genetic programs and can easily be incorporated into existing tag-enabled GP systems.

==> tex/declarations.tex <==

\vspace{0.25cm}
\noindent
\textbf{Declarations}

\begin{small}

\noindent
\textbf{Funding:} This research was supported in part by NSF grants DEB-1655715, DBI-0939454, and DGE-1424871.

\noindent
\textbf{Conflicts of interest:} The authors declare that they have no conflicts of interest.

\noindent
\textbf{Availability of data and material:} Our experimental data is publicly available as an Open Science Framework repository at \url{https://osf.io/928fx/}.

\noindent
\textbf{Code availability:} Our source code is publicly available on GitHub at \url{https://github.com/amlalejini/Tag-based-Genetic-Regulation-for-LinearGP} \cite{lalejini_supplement}.

\end{small}
